SocChain: Blockchain with Swift Proportional Governance for Bribery Mitigation

Blockchain governance is paramount to leading securely a large group of users towards the same goal without disputes about the legitimacy of a blockchain instance over another. As of today, there is no efficient way of protecting this governance against an oligarchy. This paper aims to offer a new dimension to the security of blockchains by defining the Swift Proportional Governance problem. This problem is to rapidly elect governance users that proportionally represent voters without the risk of dictatorship. We then design and implement an open permissioned blockchain called SocChain (Social Choice Blockchain) that mitigates bribery by building upon results in social choice theory. We deploy SocChain and evaluate our new multi-winner election DApp running on top of it. Our results indicate that using our DApp, 150 voters can elect a proportionally representative committee of 150 members within 5 minutes. Hence we show that SocChain can elect as many representatives as members in various global organizations.

==> alg/Algo0.tex <==
\begin{algorithm}[h!]
	\caption{Client operations\label{alg:sevm}}
	{\footnotesize
	\begin{algorithmic}[1]
	
		\Part{$\lit{balance}(\ms{account})$}\Comment{client request to retrieve the  balance of an account}
			\State Let $P$ be a set of $2t+1$ blockchain nodes \Comment{to $2t+1$ blockchain nodes}
			\ForAll{$p_j \in P$}   		
				  $\lit{send}(\lit{read}, \ms{account})$ to $p_j$ \Comment{multicast read message} \label{line:multicast}
			\EndFor
			\WUntil{received same balance response $b$ from $t+1$ distinct nodes}\label{line:enough-responses}\EndWUntil 
%			\If{$\exists b_1, b_2 \in B_1 ~|~ b_1 \neq b_2$} \label{line:detect-difference} \Comment{detect different responses}
%				\WUntil{received balance responses $B_2$ from $2t+1$ distinct nodes}\EndWUntil
%				\State $\ms{result} \gets b ~|~ b$ is the majority value among the responses in $B_2$  \label{line:different-copy}
%			\Else{}
%				 $\ms{result} \gets b ~|~ b \in B_1$ \label{line:same-copy} \Comment{pick any of the identical copies}
%			\EndIf
			\Return $\ms{b}$ \Comment{return balance} 
			\EndReturn
			
		\EndPart
		
		\Statex
	
		\Part{$\lit{send}(\ms{tx})$}\Comment{client request to send tx (e.g., smart contract invocation/upload)} \label{line:send-start}
			\State Let $p_j$ be one of the state nodes in my neighborhood  \Comment{to 1 neighbor}	
			\State $\lit{send}(\lit{write}, \ms{tx})$ to $p_j$ \Comment{best effort send of a write operation} \label{line:send-end}
		\EndPart
		
		\algstore{alg:blockchain0}
	
	\end{algorithmic}%
}%
\end{algorithm}%

==> alg/Reconfiguration-State.tex <==
\begin{algorithm}[h!]
	\caption{Reconfiguration of state nodes\label{alg:recon1}}
	{\footnotesize
	\begin{algorithmic}[1]
		\Part{Initializations}
		 %\State $A$ \Comment{Set containing the consensus committee IPs}	
		 \State $index = k$ where $k < |A|$ \Comment{index in the array of IP addresses}
		 \State $\ms{committee}$ reception occurs when smart contract emits (Alg.\ref{alg:stv}, line \ref{line:emit})
		\EndPart
		
		\Statex

		\Part{upon receiving $\ms{committee}$} \Comment{smart contract emits state event at Alg.\ref{alg:stv}, line~\ref{line:emit}} \label{line:emitevm}
%		\Part{$event\gets \lit{async} \lit{subscribe_{s}}(\ms{sc-address})$}\Comment{subscribe to committee event}
			%\If{\ms{event}}\Comment{If committee event is received}
			\State $\lit{stop}(\textsc{state-service})$\Comment{stops the state node}\label{line:stopevm}
				\ForAll{$\ms{ip} \in \ms{committee}$}\Comment{for IPs in committee}
					\State $A \gets A \cup \{\ms{ip}\}$ \Comment{add the IP address}
				\EndFor
					\State$\ms{ip}\gets \lit{choose}(A, \ms{index})$\Comment{select the IP at $index$ in the selected committee $I$}\label{line:selectIP}
					\State$\ms{index}\text{++}$\Comment{increment index so next time will select IP at $index+1$}
				\If{$\lit{has-started}(ip)$}\Comment{if the consensus service in ip has started}\label{line:isupconsensus}
					\State $\lit{start}(\lit{\textsc{state-service}})$\Comment{Start the state node}
					\State$\lit{connect}(ip)$ \Comment{network connection to the consensus node}\label{line:connect}
				\EndIf
		
%			\EndIf
		\EndPart
		
	
	\end{algorithmic}%
}%
\end{algorithm}%


==> alg/STV.tex <==
\begin{algorithm}[h!]
	\caption{Single Transferable Vote - Part 1\label{alg:stv}}
	{\footnotesize
	\begin{algorithmic}[1]
        \Part{Declarations}
        \State$Ballot_{i} = [X, Y, Z, ..]$ is the $i^{th}$ ballot $\mid$ $X,Y,Z$ are candidates
        \State$Ballot_{i}[k]$ is the $(k+1)^{th}$ preference of $Ballot_{k}$
        \State $size$ is the number of candidate preferences in a ballot
        \State $quota = (n-t)/(seats + 1)$ $\mid$ $n$ is the total number of consensus nodes of which $t$ are byzantine and $seats$ are the number of candidates that require to be elected
        \State $\ms{ballot-count}, select = 0$
        \State $threshold = n-t$
        \State $S=\{X,Y, Z, . . .\} \mid S$ is the set of candidates
        \EndPart
        \State
        \Part{$\lit{createCommittee}(Ballot_{i})$}
        \State$\ms{ballot-count} = \ms{ballot-count} + 1$
        \If{$\ms{ballot-count} = \ms{threshold}$}   \Comment{if ballots received equals threshold}
        %\ForAll{$i=0; i < \ms{ballot-count}; pref_{i}=0$}  \Comment{start from first preference}
        \ForAll{$i=0; i < \ms{ballot-count};i++$} 
        \State $\ms{pref}_{i}=0$
        \If{$Ballot_{i}$[$pref_{i}$]=$c$ $\mid c$ is in $\lit{S}$}
        votes[$c$]=votes[$c$] + 1\Comment{calculate votes for candidate $c$ for first preference}
        \EndIf
        \EndFor
        \State$round=0$
        \While{$|selected| < seats$}\Comment{do until the elected nodes equal the seats available}
        	\State$\lit{STV()}$
        	\State$round = round +1$
        	\If{$|S|-|eliminated| = seats$}\Comment{break the loop since if more are eliminated seats cannot be filled}
        		\State break
        	\EndIf
        \EndWhile
        
        \ForAll{$k=0; k< \ms{size};k++$}
        \ForAll{$i=0; i < \ms{ballot-count};i++$}
        \If{$|selected| < seats$ and
               $Ballot_{i}[k]=c \mid c$ is in $\lit{S}$, not in $\lit{selected}$ and not in $\lit{eliminated}$}
           \State $\lit{selected} \gets \lit{selected} \cup \{c\}$
        \EndIf
        \EndFor
        \EndFor
        
        \EndIf
        
        \EndPart
        
        \algstore{stv}
        
	\end{algorithmic}%
}%
\end{algorithm}%
\begin{algorithm}[h!]
	\caption{Single Transferable Vote - Part 2\label{alg:stv1}}
	{\footnotesize
	\begin{algorithmic}[1]
	
        \algrestore{stv}
        
        \Part{$\lit{STV}()$}
        \If{$\exists c \mid \lit{votes[c]} \geq quota$}\Comment{if the quota is equalled or exceeded}
         \State $\lit{selected} \gets \lit{selected} \cup \{c\}$\Comment{elect candidate}
        \If{$\lit{votes[c]} > quota$}
        	\State $\ms{excess-candidates}\gets \ms{excess-candidates} \cup \{c\}$\Comment{save candidates that exceed quota in $\ms{excess-candidates}$}
            \State$\ms{excess-vote_{c}} \gets \lit{votes[c]} - quota$\Comment{excess vote from candidate $c \mid c \exists$ in $\lit{S}$}
        \EndIf
        
        \State $\forall i$ 
        \If{$Ballot_{i}[pref_{i}]=c$ and $c \in \ms{excess-candidates}$}\Comment{If the current preference of the ballot is one of the excess candidates}
        \State$\ms{count{c}} \gets \ms{count_{c}} + 1$\Comment{The number of candidates $c$}
        $\ms{pref-next}_{i} \gets \ms{pref}_{i} + 1$
        \While{$Ballot_{i}[\ms{pref-next}_{i}] \not\in (selected \cup eliminated$)}\Comment{Increment the preference pointer until a non eliminated non selected candidate is found}
        \State $\ms{pref-next}_{i} \gets \ms{pref-next}_{i} + 1$
        \EndWhile
        %\State $\ms{pref-next}_{i} \gets \ms{pref}_{i} + 1$ %\Until{$Ballot_{i}[\ms{pref-next}_{i}] \not\in selected \not\in eliminated$}
        
        \If{$Ballot_{i}[pref_{i}]=c$ and $c \in \ms{excess-candidates}$ and $Ballot_{i}[\ms{pref-next}_{i}] \not\in  \lit{selected} \cup \lit{eliminated}$}
        \State $\ms{pref_{i}} =\ms{pref-next}_{i}$\Comment{move the preference pointer}
        \State $z \gets Ballot_{i}[\ms{pref}_{i}]$
        \State $candidates-next \gets candidates-next \cup (c,z)$\Comment{A tuple of the current candidate and the next candidate} 
        \State$\ms{count_{z}} \gets \ms{count_{z}} + 1$\Comment{The number of candidates $z$}
        \EndIf
        \EndIf
        
        \ForAll{unique $(c,z) \in \ms{candidates-next}$}
        \State$\lit{vote(z)} \gets \lit{vote(z)} + \ms{excess-vote_{c}} \cdot (count_{z}/\ms{count{c}})$\Comment{transfer excess votes to the next valid preference of the ballots}
        \EndFor
        
        \EndIf
         %\EndIf
        
        \If{$\forall c : votes[c] < quota$}\Comment{There are no candidates reaching the quota in the round}
        \State $\ms{eliminated} \gets \ms{eliminated} \cup t \mid t = \lit{min_{\forall c}(votes[c])}$\Comment{eliminate the candidate with the least votes}
        \State $\ms{transfer-vote} \gets \lit{votes[t]}$
        \State $\lit{votes[t] \gets 0}$\Comment{Assign votes of least candidate to 0}
         \ForAll{$k=0; k<size;k++$}
         	\ForAll{$i=0; i < \ms{ballot-count};i++$}
         		\If{$Ballot_{i}[k]=t$}
         			$elimpointer \gets elimpointer\cup (i,k)$\Comment{Store tuples of ballot number and preference index that references least voted candidate}
         		\EndIf
         	\EndFor
         \EndFor
         
         \If{$\exists (v,k) \in elimpointer \mid Ballot_{v}[k]=m$ and $m \in \ms{eliminated}$}\Comment{If the preference $k$ of the ballot $v$ is eliminated}
         \State $\ms{pref-next}_{v}=k+1$
         \State $\ms{count{m}} \gets \ms{count_{m}} + 1$\Comment{The number of candidates $m$}
         \While{$Ballot_{v}[pref-next_{v}] \not\in (selected \cup eliminated)$}\Comment{Increment the preference pointer until a non eliminated non selected candidate is found}
         \State $\ms{pref-next}_{v} \gets \ms{pref-next}_{v} + 1$
         \EndWhile
         %\Until{$Ballot_{v}[pref-next_{v}] \not\in selected \not\in eliminated$}
         
         \If{$Ballot_{v}[\ms{pref-next}_{v}] \not\in  \lit{selected} \cup \lit{eliminated}$}
         \State $pref_{v}\gets \ms{pref-next}_{v}$\Comment{move the preference pointer}
         \State $z \gets Ballot_{i}[\ms{pref}_{v}]$
         \State $candidates-next \gets candidates-next \cup (m,z)$\Comment{A tuple of the least voted candidate and the next candidate in ballot} 
         \State$\ms{count_{z}} \gets \ms{count_{z}} + 1$\Comment{the number of candidates $z$}
         \EndIf
         \EndIf
        
        \ForAll{unique $(m,z) \in candidates-next$}
        \State$\lit{vote(z)} \gets \lit{vote(z)} + \ms{transfer-vote} x (\ms{count_{z}}/\ms{count_{m}})$\Comment{transfer votes from the least voted candidate to next preference in their ballots.}
        \EndFor
        
        \EndIf
        \EndPart
	
	\end{algorithmic}%
}%
\end{algorithm}%
